New sensitivity of current LHC measurements to vector-like quarks

Quark partners with non-chiral couplings appear in several extensions of the Standard Model. They may have non-trivial generational structure to their couplings, and may be produced either in pairs via the strong and EM interactions, or singly via the new couplings of the model. Their decays often produce heavy quarks and gauge bosons, which will contribute to a variety of already-measured "Standard Model" cross-sections at the LHC. We present a study of the sensitivity of such published LHC measurements to vector-like quarks, first comparing to limits already obtained from dedicated searches, and then broadening to some so-far unstudied parameter regions.

==> mkgenplots <==
#! /usr/bin/env bash

ROOT=$PWD
test "$GENS" || GENS=123
test "$STYLE" || STYLE=final

function mkplots() {
    FILE=$(basename $MAP)
    DIR=$(dirname $MAP)
    cd $DIR
    echo "In $PWD..."
    if [[ -e $FILE ]]; then
        echo $PWD && contur-plot $FILE mtp $KNAME -x '$M_Q$ (GeV)' -y '$\kappa$' --style=$STYLE -o . $@
    else
        echo "No contur.map file found" 1>&2
    fi
    echo
}

(echo $GENS | grep -q 1) && {
    echo "Generation 1"
    MAP=$ROOT/1Gen/HWZ001/contur.map GEN=1 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/1Gen/HWZ010/contur.map GEN=1 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/1Gen/HWZ100/contur.map GEN=1 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/1Gen/HWZ111/contur.map GEN=1 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    echo
    wait
}

(echo $GENS | grep -q 2) && {
    echo "Generation 2"
    MAP=$ROOT/2Gen/HWZ001/contur.map GEN=2 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/2Gen/HWZ010/contur.map GEN=2 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/2Gen/HWZ100/contur.map GEN=2 KNAME=KT mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/2Gen/HWZ111/contur.map GEN=2 KNAME=KT mkplots -d $ROOT/flavlimits.py &
    echo
    wait
}

(echo $GENS | grep -q 3) && {
    echo "Generation 3"
    MAP=$ROOT/3Gen/HWZ001/contur.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ010/contur.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ100/contur.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ111/contur.map GEN=3 KNAME=KT mkplots &
    echo
    wait

    echo "Generation 3 no-correlations"
    MAP=$ROOT/3Gen/HWZ001/nocorr/conturNoCorr.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ010/nocorr/conturNoCorr.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ100/nocorr/conturNoCorr.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ111/nocorr/conturNoCorr.map GEN=3 KNAME=KT mkplots &
    wait
}

